ILC Reference Design Report Volume 4 - Detectors

This report, Volume IV of the International Linear Collider Reference Design Report, describes the detectors which will record and measure the charged and neutral particles produced in the ILC's high energy e+e- collisions. The physics of the ILC, and the environment of the machine-detector interface, pose new challenges for detector design. Several conceptual designs for the detector promise the needed performance, and ongoing detector R&D is addressing the outstanding technological issues. Two such detectors, operating in push-pull mode, perfectly instrument the ILC interaction region, and access the full potential of ILC physics.

==> subsystems/beamcal.tex <==
\section{BeamCAL}
Draft 0 Outline, 20 Sept 2006\\
R. Frey, primary author

\subsection{Introduction}
Raison d'etre: angular coverage – 2 detectors, BeamCal and PhotoCal/GamCal;
physics (electron veto/hermeticity in BeamCal) and accelerator functions
(beamstrahlung in GamCal and BeamCal)
Environment: backgrounds and radiation; crossing angles

\subsection{Technology options}
BeamCal: W/diamond, W/GaAs, W/silicon;
GamCal: converter + Cherenkov, gas jet + magnet + converter, converter + TRD,
?? ;
Technology and simulation studies cut across the Concepts: FCal

\subsection{ Current status and R\&D challenges}
Current: Full simulation studies, including beam backgrounds, are well advanced.
More effort needed for detector development/tests. Recent tests of sensors.

\subsection{Challenges}
BeamCal Develop/test detector technology and detector configuration for a very
hostile environment; issues include radiation hardness, detector stability, fast
active readout material, fast electronic readout, 3 MHz feedback to accelerator.
High occupancy and position requirement imply high granularity.
Single electron veto in enormous low-energy background implies large dynamic
range.
Design goals must be re-evaluated for various IR beam-crossing angle
configurations.

GamCal: Find acceptable design and technology; 3 MHz feedback to accelerator;
how to separate pairs and photons - IR configuration dependent

\subsection{Milestones}
Next 1-2 years: Establish viable detector technology; evaluate with test beams.
1-2 years: Establish mechanical designs for specific Concept and IR configurations.

==> subsystems/magnet-0804.tex <==
\section{Superconducting Detector Magnets for ILC}
\label{sec-subs-magnet}

%\subsection{Introduction}
The use of magnetic fields is a fundamental method to analyze the momentum of charged particles.  In order to extend the energy 
range in particle physics, large-scale magnetic fields are inevitably required.  The basic relation between magnetic field strength, 
charged particle momentum, and bending radius is described with $p = \gamma mv = q \rho B$ where $p$ is the momentum, $m$ the mass, $q$ the charge, $\rho$ 
the bending radius, and $B$ the magnetic field.  The deflection (bending) angle, $\phi$, and the sagitta,$s$, of the trajectory 
are determined by;
\begin{equation}
   \phi	\approx L / \rho = q B L / p, \ \ \ {\rm and} \ \ \ 
      s \approx q B L^2 / 8 p   \label{eq-subs-magnet1}
\end{equation}
where $L$ is the path length in the magnetic field. For practical measurements in high energy colliding beam detectors, both field strength
and magnetic volume have been increased. A general-purpose detector consists of three major stages:  a central tracker 
close to the interaction point, a set of electromagnetic and hadronic calorimeter systems, and an external muon detector system.  
The momentum measurement is carried out in the region of the tracker, although it may be augmented for muons in the muon detector,
and requires a powerful magnetic field to achieve high resolution.

   The solenoid field has been widely used in many colliding experiments \cite{ref-mag1,ref-mag2,ref-mag3,ref-mag4,ref-mag5,ref-mag6}.  It features uniform field in the axial direction with self-supporting structure.  
%On the other hand, the charged particle inevitably passes through the solenoidal coil as part of the detector system. 
%Therefore, material used in the coil and the cryostat required to be minimized, especially at the solenoid coil placed
%in front of the electromagnetic calorimeters.  
The magnetic flux needs to return outside the solenoid coil, and in most cases, an iron yoke provides the flux return.  An external solenoid with the reversed field may also provide flux return, and it requires a much more sophisticated magnet system in terms of stored energy, quench protection and mechanical support. 

   The momentum analysis is usually performed by measurement of particle trajectories inside the solenoid, and the momentum resolution 
is expressed by
\begin{equation}
   \sigma_p/p \approx  p / (B • L^2) \label{eq-subs-mag2}
\end{equation}	
where $L$ corresponds to the solenoid coil radius, $R$.  Therefore, a larger coil radius may be an efficient approach to reach better 
momentum resolution, although overall detector cost considerations must also be taken into account. In this section progress in the 
design of solenoidal detector magnets 
is reviewed, and possible detector magnet design for 
the International Linear Collider (ILC) experiments are discussed. 


\subsection{Progress in superconducting detector solenoid magnets} 
   Table~\ref{tab-mag1} lists progress of the superconducting solenoids in collider experiments~\cite{ref-mag1}. The CDF solenoid 
established a fundamental technology of the ``co-extruded aluminum stabilized superconductor"~\cite{ref-mag7} which has become a 
standard for the detector magnet based on the pioneer work for the colliding beam detector solenoid at ISR ~\cite{ref-mag8} and 
CELLO \cite{ref-mag9}.  The TOPAZ solenoid established the ``inner winding'' technique to eliminate the inner coil 
mandrel \cite{ref-mag10}.  The ALEPH solenoid demonstrated indirect and thermo-syphon cooling for stable cryogenics operation 
in large scale detector magnets~\cite{ref-mag11}. In the SDC prototype solenoid, the mechanical reinforcement of 
aluminum-stabilized superconductor was further developed \cite{ref-mag12}. In the LHC project at CERN, two large superconducting 
magnet systems have been developed for ATLAS and CMS with extensive efforts for the high-strength aluminum stabilized superconductor. 

   The magnetic field design of the ATLAS detector is composed of an axial field by using a solenoid coil in the central region and of an azimuthal field by using a set of toroidal coils~\cite{ref-mag13}.  Since the solenoid coil is placed in front of the liquid-argon calorimeter, it is required to be as thin and transparent as possible to achieve the best calorimeter performance. Therefore, the solenoid coil was designed with features (1) high-strength aluminum stabilized superconductor  uniformly reinforced, (2) pure-aluminum strip technique for uniform energy absorption and quench protection, and (3) a common cryostat with the LAr calorimeter to ultimately save magnet wall-material. Extensive efforts have been made to reinforce the aluminum stabilizer while keeping adequate low electrical resistivity as discussed below~\cite{ref-mag14}.  

   The CMS detector is designed as a single solenoidal magnet surrounded by the iron return yoke~\cite{ref-mag15, ref-mag16, ref-mag17}.  Special effort has been made to reinforce the aluminum stabilized superconductor in a hybrid configuration as discussed below~\cite{ref-mag18}.  

{\footnotesize{
\begin{table}[thb]
  \caption{\label{tab-mag1}Progress of detector solenoid magnets in high energy physics.}
\begin{footnotesize}
\begin{tabular}{ll|cccccc}
\hline
Name & Laboratory &B & R & L & E & X  & E/M  \\
           &     & [T]  & [m] & [m] &       [MJ]   & [$x_0$] & [kJ/kg] \\
\hline
CDF& Tsukuba/FNAL& 1.5&1.5&5.07&30&0.84&5.4\\
TOPAZ$^*$ & KEK & 1.2& 1.45& 5.4& 20& 0.70& 4.3\\
VENUS$^*$ & KEK& 0.75& 1.75& 5.64& 12& 0.52& 2.8\\
AMY$^*$ & KEK& 3& 1.29& 3& 40& $\#$ & \\ 
CLEO-II&Cornell&1.5&1.55&3.8&25&2.5&3.7\\
ALEPH$^*$&Saclay/CERN&1.5&2.75&7.0&130&2.0&5.5\\
DELPHI$^*$&RAL/CERN&1.2&2.8&7.4&109&1.7&4.2\\
ZEUS & INFN/DESY& 1.8& 1.5& 2.85&11&0.9&5.5\\
H1&RAL/DESY&1.2&2.8&5.75&120&1.8&4.8\\
BABAR& INFN/SLAC& 1.5& 1.5& 3.46& 27& $\#$ & 3.6\\
D0 & Fermi& 2.0& 0.6& 2.73& 5.6& 0.9& 3.7\\
BELLE&KEK&1.5&1.8&4&42&$\#$&5.3\\
BES-III$+$&IHEP&1.0&1.45&3.5&9.5&$\#$&2.6\\
ATLAS & & & & & & & \\
~~~Central&ATLAS/CERN&2.0&1.25&5.3&38&0.66&7.0\\
~~~Barrel &ATLAS/CERN&1&4.7-9.7&5&26&1080&  \\
~~~Endcap &ATLAS/CERN&1&0.825-5.35&5&2 $\times$ 250&-&\\
CMS$+$ &CMS/CERN&4&6&12.5&2600&$\#$&12\\
\hline
\multicolumn{8}{l}{$^*$ operation complete}\\
\multicolumn{8}{l}{$+$detector under construction}\\
\multicolumn{8}{l}{$\#$EM calorimeter inside solenoid, so small radiation length, X, not a goal}\\
\end{tabular}
\end{footnotesize}
\end{table}
}}

\subsection{Progress of Aluminum Stabilized Superconductor}
Aluminum stabilized superconductor represents a major technological advance in detector magnets. It has been developed to provide large-scale magnetic fields with minimum material~\cite{ref-mag5}.  In Figure~\ref{fig-mag1} cross-sectional vviews of aluminum stabilized superconductors are shown for various generations of detector magnets used high-energy physics experiments.  
\begin{figure}
	\centering
		\includegraphics[width=12cm]{subsystems/magnet_history.eps}
	\caption[Development of aluminum stabilized superconductors in particle physics.]
{Cross sectional view of aluminum stabilized superconductors
which have been used for different collider detector magnets.
The conductors are arranged chronologically from left to right.
A scale is indicated by the double arrow in the center of the figure.}
	\label{fig-mag1}
\end{figure}
Major progress on the mechanical properties of the conductor has been achieved by using a 
NbTi/Cu superconductor co-extruded with an aluminum stabilizer by diffusion bonding. One approach consists of a ''uniform reinforcement''~\cite{ref-mag5}, and the other consists of a ``hybrid configuration''~\cite{ref-mag18}. The uniform reinforcement was made, in the SDC and ATLAS solenoid, by ``micro-alloying'' followed by ``cold-work hardening''~\cite{ref-mag19}. By this the strength of the aluminum stabilizer could be much improved while the excellent electrical properties were retained without increasing the material.   Another technical approach for the reinforcement has been made, in the CMS solenoid, by using a hybrid (or block) configuration, which consists of pure-aluminum stabilized superconductor and high strength aluminum alloy (A6082) blocks at both ends fixed by using electron-beam welding.  The hybrid configuration is very useful and practical in large-scale conductors~\cite{ref-mag20, ref-mag21}.
          
   Based on these successful developments of both ``uniform reinforcement'' and ``hybrid configuration'' further improvement has been proposed, for future applications, in combining these efforts~\cite{ref-mag21,ref-mag22} as summarized in Table~\ref{tab-mag2}, and shown in Figure~\ref{fig-mag2}.  The central part of the CMS conductor partly composed of pure-aluminum stabilizer may be replaced by a Ni-doped high strength aluminum stabilizer developed for the ATLAS solenoid. This may result in a further reinforcement of the overall aluminum stabilized superconductor. It may be applicable in the ILC detector magnets especially for the high field magnet such as the SiD solenoid discussed later.  
{{   
\begin{table}[thb]
\caption[High-strength aluminum stabilized superconductors]{\label{tab-mag2}{Progress of high-strength aluminum stabilized superconductor and possible future upgrade.}}
\begin{center}
\begin{footnotesize}
\begin{tabular}{ll|lccc}
\hline
     & Reinforced  &Feature        &Aluminum        &Full cond       & Full cond \\ 
     &             &               &\multicolumn{2}{c}{yield strength} & RRR \\
\hline
\multicolumn{2}{l}{\underline{Progress at LHC}}&&&\\
ATLAS&  Uniform & Ni(0,5 \%)-Al    & 110      & 146      &        590 \\
CMS  & Hybrid   & Pure-Al\&A6082-T6& 26 / 428 & 258      & $\sim$ 1400 \\
\hline
\multicolumn{2}{l}{\underline{Improvements for ILC}}&&&\\
     & Hybrid   & Ni-Al\& A6082-T6 & 110 / 428 & $\sim$ 300 & $\sim$ 300\\
     & Hybrid   & Ni-Al\& A7020-T6 & 110 /677  & $\sim$ 400  & $\sim$ 300\\
\hline
\end{tabular}
\end{footnotesize}
\end{center}
\end{table}
}}

\begin{figure}
	\centering
		\includegraphics[height=3cm]{subsystems/magnet_conductor.eps}
		\caption[Possible hybrid magnet configurations]{Possible hybrid magnet conductor configurations based on technologies established for 
the LHC detector magnets.}
	\label{fig-mag2}
\end{figure}

\subsection{$\bf E/M$ ratio as a Performance Measure}
The ratio of stored energy to cold mass ($E/M$) in a superconducting magnet is a useful performance measure. In an ideal solenoid with a perfect axial field, it is also expressed by a ratio of the (hoop) stress, $c_h$, to the average 
density, $d$~\cite{ref-mag1,ref-mag5}:
\begin{equation}
\label{eq-subs-mag3}
%   E/M	=\left\{ \int{ B^2/2 {\mu_0}  d\nu \right\} / \left{ d \cdot V_{coil}} \right\}  \approx c_h / 2d .
   E/M	\approx c_h / 2d.
\end{equation}

Figure~\ref{fig-ratio} shows the E/M ratio in various detector magnets in high energy physics.  Assuming an approximate average density of $3\times10^3 $kg/m$^3$ for the conductor, and an E/M ratio of $10$~kJ/kg, the hoop stress level will be $\sim 60$~MPa. In the case of an iron free solenoid, the axial stress, $\sigma_z$, will be one half of the hoop stress, and the stress intensity $(c_h + c_z)$ then is around $90$~MPa. This has to be sufficiently lower than yield strength of the coil material, in a mechanically safe design.

\begin{figure}
	\centering
		\includegraphics[height=8cm]{subsystems/magnet_energy.eps}
	\label{fig-ratio}
	\caption{Ratio E/M of stored energy to cold mass for existing thin detector solenoids}
\end{figure}

	The E/M ratio in the coil is approximately equivalent to the enthalpy of the coil, $H$. It determines the average coil temperature rise after energy absorption in a quench:
\begin{equation}
\label{eq-subs-mag4}
   E/M = H (T_2) - H (T_1) \approx  H (T_2), 
\end{equation}
where $T_2$ is the average coil temperature after the full energy has been absorbed in a quench, and $T_1$ is the initial temperature. E/M ratios of 5, 10 and 20~kJ/kg correspond to $\sim 65$ , $\sim 80$, and $\sim 100$~K temperature rise, respectively. The E/M ratios in various detector magnets are shown in Figure~\ref{fig-ratio} as a function of the total stored energy. The CMS magnet has the 
currently largest E/M ratio at $12$~kJ/kg as well as the largest stored energy. In the case of a quench, 
the protection system at CMS has been designed to keep the temperature below $80$~K.

In developing a high field magnet, the limiting factor usually is the temeprature increase the 
coil can tolerate in case of a quench. This would favour high mass coils, contrary to 
the requirements on a light coil expressed by all experiments. 
%One would like the cold mass to be as small as possible to minimize the material in the coil as well as to maximize the field strength, but temperature rise during a quench must also be minimized.   The E/M ratio as large as $12$~kJ/kg is designed in the CMS solenoid, with assuming about a half of the stored energy to be extracted to the external dump resistor. So the coil temperature can be kept below 80 K, under the condition of the energy extraction system functioning well. The coil design is usually limited by the maximum temperature rise  that the coil can tolerate during the coil quench. This maximum temperature would be set to $< 130 K (50 K + 80 K)$, so that thermal stress effects in the coil are manageable. 
The success of the CMS solenoid suggests that the E/M ratio of the detector magnet design in the ILC experiment as large as 12 kJ/kg or even slightly higher can be tolerated. 
It may help to design the higher field magnet with larger stored energy.  It should also be noted that a higher E/M ratio would be required to realize much higher field and/or much larger-scale superconducting magnets for the ILC detector magnets as discussed below.


\subsection{Detector Magnets at the ILC} 
According to the ILC detector outline documents~\cite{ref-GLD,ref-LDC,ref-SiD,ref-4th}, the detector magnet design requirements are 
listed in Table~\ref{tab-mag3}, and are compared with the LHC detector solenoids successfully commissioned.  

\begin{table}[tbh]
\caption[Detector Solenoids at LHC and ILC]{\label{tab-mag3}Superconducting detector solenoids for ILC compared with detector solenoids at LHC.}

\begin{footnotesize}
\begin{tabular}{ll|ll|lllll}
\hline
Parameters& unit & \multicolumn{2}{c}{LHC} & \multicolumn{5}{c}{ILC}\\
\hline
& & ATLAS& CMS& GLD& LDC& SiD& \multicolumn{2}{c}{4th}\\
& & \multicolumn{1}{c}{CS} & & & & & Inner & Outer \\ 
\hline
\multicolumn{2}{l|}{\bf Basic requirements}&&&&&&\\
\hline
Clear-bore radius      & m     &7    & 1.18  & 4.00  &3.00   & 2.5     & 3.0   &     \\
Central magnetic field & Tesla & 2   & 4     &3      & 4     & 5    &3.5   & 1.5 \\
\hline
\hline
\multicolumn{2}{l|}{\bf Design parameters}&&&&&&\\
\hline
Coil inner radius      & m     & 1.23 & 3.25  & (4.0) &	3.16  &2.65 & 3   & 5.4\\
Coil half length       & m     & 2.7  &6.25   & 4.43  & 3.3   & 2.5 & 4   & 5.5\\
Coil layers            &       & 1    &4      & 2     &4      & 6   &     & \\
Cold mass thickness    & m     & 0.04 & 0.3   & 0.4   &  0.3  & 0.4 &     & \\
Maximum field in coil  & Tesla & 2.6  & 4.6   & 3.5   &  4.6  & 5.8 &     & \\
Nominal current        & kA    & 7.73 & 20    &       &       & 1.8 &     & \\
Stored energy          & GJ    & 0.04 & 2.6   & 1.6   & 1.7   & 1.4 & 5.7 & \\
Cold mass weight       & ton   & 5.7  & 220   & 78    & 130   &     &     & \\
E/M                   & kJ/kg & 7    & 12.3  & 20    & 13    & 12  &     & \\
\hline
Reference&  & \cite{ref-mag12}& \cite{ref-mag15} & \cite{ref-GLD} & \cite{ref-LDC} & \cite{ref-SiD,ref-mag27}  & \multicolumn{2}{c}{\cite{ref-4th}} \\
\hline
\end{tabular}
\end{footnotesize}
\end{table}




\begin{figure}
	\centering
		\includegraphics[height=8cm]{subsystems/magnet_load.eps}
	\caption[Load lines for different magnet designs.]{The load line (solid line) and the critical current as a function of
the magnetic field (dashed line) of the proposed SiD superconductor(green)
and of the CMS magnet(red).  The operation point
of the SiD magnet and the CMS magnets are shown by a green square symbol
and a red diamond symbol, respectively.  The numbers in \%
are loads relative to their (mechanically) critical loads.}
	\label{fig-mag4}
\end{figure}

The development of the ILC magnets will profit heavily from the LHC experiences. The CMS magnet 
concept is the basis for the proposed ILC magnets. The GLD detector solenoid will require a larger cold mass because of the larger coil 
radius resulting in more stored energy per length.  The LDC magnet design is most similar to the CMS solenoid design.  
The SiD detector solenoid will be most challenging with the high field of 5 T resulting in larger mechanical stress and increased stored 
energy.  The smaller coil radius may help to manage the mechanical stress~\cite{ref-mag27}. Figure~\ref{fig-mag4} shows the ratio between 
actual mechanical load and the critical load for the CMS and the SiD solenoids. For SiD, it is $67 \%$ of the critical load. 
Combining the advanced superconductor technology of ATLAS and CMS may help to make the GLD and SiD solenoids more stable and reliable. 
Advances in technology may also reduce the thickness 
of all proposed coils at the ILC.

Future advances in superconducting technology may make it possible to push the limits on E/M as 
high as $15 \sim 20$~hJ/kg, which could result in either more powerful or thinner 
magnets for the ILC. Further aggressive conductor development is crucial if 
these goals should be met. 


\subsection{Summary and Outlook}
  	Based on the recent experience in the superconducting detector magnets at LHC, the ILC detector magnets will be designed as follows:

\begin{enumerate}
\item The magnet will use high-strength aluminum stabilized superconductor as used in the ATLAS and CMS solenoids. The magnet technology developed for the CMS solenoid can be applied and extended.   
\item The conductor mechanical strength may be further improved by combining both features of the high-strength aluminum stabilizer (Ni-doping and cold-work reinforcement) developed for the ATLAS solenoid and ``hybrid configuration'' reinforced by high-strength aluminum alloy placed at both ends of the coil developed for the CMS solenoid.   
\item High $E/M$ ratios in the cold mass has been reached by CMS and it does seem possible to achieve even higher E/M ratio up to 20~kJ/kg, depending on the required magnetic field and compactness of the magnet design. 
\item A highly redundant and reliable safety system needs to be an integral part of 
any magnet design, to protect the magnet in case of quench. Energy extraction should be the primary protection scheme and fast 
quench trigger, which initiates a heater induced quench, should be an important backup system.  
\end{enumerate}

	A special effort will be required to realize the 4th detector design. It will require major efforts in mechanical design as well
 as in the magnet safety design because of the extraordinary large electromagnetic force (and de-centering force), stored energy and 
the resulting mechanical complexity.  A sophisticated mechanical design and engineering work will be required. 	

	In the long range future, even higher field solenoids might be feasible by pushing $E/M > 20$~kJ/kg.  Such a design may be 
realized with further improvements in the conductor, with significantly larger yield strength. 
	
